Neural Architecture Search as Multiobjective Optimization Benchmarks: Problem Formulation and Performance Assessment

The ongoing advancements in network architecture design have led to remarkable achievements in deep learning across various challenging computer vision tasks. Meanwhile, the development of neural architecture search (NAS) has provided promising approaches to automating the design of network architectures for lower prediction error. Recently, the emerging application scenarios of deep learning have raised higher demands for network architectures considering multiple design criteria: number of parameters/floating-point operations, and inference latency, among others. From an optimization point of view, the NAS tasks involving multiple design criteria are intrinsically multiobjective optimization problems; hence, it is reasonable to adopt evolutionary multiobjective optimization (EMO) algorithms for tackling them. Nonetheless, there is still a clear gap confining the related research along this pathway: on the one hand, there is a lack of a general problem formulation of NAS tasks from an optimization point of view; on the other hand, there are challenges in conducting benchmark assessments of EMO algorithms on NAS tasks. To bridge the gap: (i) we formulate NAS tasks into general multi-objective optimization problems and analyze the complex characteristics from an optimization point of view; (ii) we present an end-to-end pipeline, dubbed $\texttt{EvoXBench}$, to generate benchmark test problems for EMO algorithms to run efficiently -- without the requirement of GPUs or Pytorch/Tensorflow; (iii) we instantiate two test suites comprehensively covering two datasets, seven search spaces, and three hardware devices, involving up to eight objectives. Based on the above, we validate the proposed test suites using six representative EMO algorithms and provide some empirical analyses. The code of $\texttt{EvoXBench}$ is available from $\href{https://github.com/EMI-Group/EvoXBench}{\rm{here}}$.

==> 9-bios.tex <==
\newpage

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.2in,clip,keepaspectratio]{figures/bios/zhichao-lu-full-shaded}}]{Zhichao Lu} received his Ph.D. degree in Electrical and Computer Engineering from Michigan State University, USA, in 2020. He is currently an Assistant Professor in School of Software Engineering at Sun Yat-sen University, China.  His current research focuses on the intersections of evolutionary computation, learning, and optimization, notably on developing efficient, reliable, and automated machine learning algorithms and systems. He received the GECCO-2019 best paper award. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.2in,clip,keepaspectratio]{figures/bios/RanCheng.eps}}]{Ran Cheng} (M'16-SM'22)
received the B.Sc. degree from the Northeastern University, Shenyang, China, in 2010, and the Ph.D. degree from the University of Surrey, Guildford, U.K., in 2016.He is currently an Associate Professor with the Department of Computer Science and Engineering, Southern University of Science and Technology, Shenzhen, China.He is a recipient of the 2018 and 2021 IEEE Transactions on Evolutionary Computation Outstanding Paper Award, the 2019 IEEE Computational Intelligence Society (CIS) Outstanding Ph.D. Dissertation Award, and the 2020 IEEE Computational Intelligence Magazine Outstanding Paper Award. He is the founding Chair of the IEEE CIS Shenzhen Chapter. He is an Associate Editor of the IEEE TEVC, the IEEE TAI, and the IEEE TCDS.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.2in,clip,keepaspectratio]{figures/bios/YaochuJin.eps}}]{Yaochu Jin} (M'98-SM'02-F'16) 
received the B.Sc., M.Sc., and Ph.D. degrees from Zhejiang University, Hangzhou, China, in 1988, 1991, and 1996, respectively, and the Dr.-Ing. degree from Ruhr University Bochum, Germany, in 2001.
He is presently an Alexander von Humboldt Professor for Artificial Intelligence, Chair of Nature Inspired Computing and Engineering, Faculty of Technology, Bielefeld University, Germany, and a Distinguished Chair in Computational Intelligence, Department of Computer Science, University of Surrey, Guildford, U.K.
His main research interests include data-driven evolutionary optimization, trustworthy machine learning, multiobjective evolutionary learning, and evolutionary developmental systems.
Prof. Jin is the Editor-in-Chief of Complex \& Intelligent Systems.He was the Editor-in-Chief of the IEEE TCDS and the Vice President for Technical Activities of the IEEE Computational Intelligence Society. He is named as a Highly Cited Researcher for 2019, 2020 and 2021 by the Web of Science Group. He is a Fellow of IEEE and a Member of the Academia Europaea.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.2in,clip,keepaspectratio]{figures/bios/KayChenTan.eps}}]{Kay Chen Tan}  (Fellow, IEEE) received the B.Eng. degree (with First Class Hons.) and the Ph.D. degree from the University of Glasgow, Glasgow, U.K., in 1994 and 1997, respectively. He is currently a Chair Professor with the Department of Computing, The Hong Kong Polytechnic University, Hong Kong. He was the Editor-in-Chief of IEEE TRANSACTIONS ON EVOLUTIONARY COMPUTATION, and is currently the Editorial Board Member of more than ten journals. He is also the Vice-President (Publications) of IEEE Computational Intelligence Society, IEEE Distinguished Lecturer Program (DLP) speaker, Honorary Professor with the University of Nottingham, Nottingham, U.K., and the Chief Co-Editor of Springer Book Series on \textit{Machine Learning: Foundations, Methodologies, and Applications}. 
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.2in,clip,keepaspectratio]{figures/bios/kdeb.png}}]{Kalyanmoy Deb} 
is University Distinguished Professor and Koenig Endowed Chair Professor at the Department of Electrical and Computer Engineering at Michigan State University (MSU), East Lansing, USA. Prof. Deb's research interests are in evolutionary optimization algorithms and application in optimization and machine learning. He is a fellow of IEEE and ASME. He has written more than 580 research papers and received many awards including Infosys prize and Edgeworth Pareto award. 
\end{IEEEbiography}


